Rewrite it in Rust: A Computational Physics Case Study

Surveys of computational science show that many scientists use languages like C and C++ in order to write code for scientific computing, especially in scenarios where performance is a key factor. In this paper, we seek to evaluate the use of Rust in such a scenario, through implementations of a physics simulation in both C++ and Rust. We also create a parallel version of our Rust code, in order to further explore performance as well as parallel code complexity. Measuring performance as program runtime, we find that Rust can offer better performance than C++, with some test cases showing as much as a 5.6$\times$ performance increase, and that parallel code in Rust can further improve performance while being easy to write safely. Finally, we provide some preliminary profiling to better understand the difference between the way our implementations perform.

==> old-sections/abstract.tex <==
% !TEX root = main.tex 

==> old-sections/background.tex <==
% !TEX root = main.tex 

\section{Background}
\subsection{The CBET Problem}
% *definitely* need to cite some sources here.
% Basing this off of what I was told for the motivation of the CBET project, could probably use a great deal of improvement?
Researchers worldwide are studying fusion energy for its potential to be a clean and virtually unlimited source of electricity and industrial heat in the future.
For laser-driven fusion studies, one of the biggest challenges is to model various factors that affect the fusion efficiency, including the Cross Beam Energy Transfer (CBET) effect.
CBET is an interaction that happens when multiple laser beams intersect in plasma. When they intersect, they can interact with plasma waves and a certain amount of energy can be transferred from one beam to another; the same concept generalizes from two beams to N beams intersecting.
A fast and accurate simulation of this interaction is crucial in building a simulator of laser systems.
While the use of experimental laser systems is in high demand, they are expensive to operate and slow, so building a fast and accurate simulator would make it easier for scientists to design experiments to run on laser systems, advancing the speed with which research can be done on them.

% I'm doing a lot of guessing here please help
The CBET program represents the plasma-filled space that the laser beams pass through as a mesh, which discretizes the space into small regions called zones. Each zone of the mesh corresponds to a specific subsection of the space, and carries information about that space, such as its electron density. The presence of an electron density gradient in space causes the rays to refract (i.e. change direction) within the plasma. Laser beams are represented as a set of discrete rays, with each ray's trajectory represented as a list of crossings between that ray and the zones of the mesh. Each crossing stores the intensity of that ray at that crossing.

The following is a short summary of the simulator code:
\begin{enumerate}
    \item Create the mesh, beams, and rays.
    \item Trace the rays: for each ray, follow its trajectory and save the location of each crossing of the mesh. Set the intensity of each crossing to the initial intensity of the laser beam.
    \item Calculate the CBET interaction multiplier: each pair of crossing rays from different beams is allowed to exchange energy according to an equation governing the interaction \cite{Follett+:PRE18}.
    \item Update the intensities: modify the ray intensities for the downstream portions of the trajectories for the crossing rays. Each crossing results in one of the rays increasing in intensity and the other decreases.
    \item Repeat the previous two steps until the change in intensity is smaller than a user-prescribed ``convergence" constant. Typically a relative change of $10^{-3}$ to $10^{-4}$ is sufficient.
%    \begin{enumerate}
%        \item For each crossing, use its intensity and the intensities of the crossings of the other beams in the same zone (if there are any) to calculate an interaction multiplier.
%        \item For each ray, update the intensity at each crossing, using those interaction multipliers
%    \end{enumerate}
    \item Calculate the average intensity value of all of the crossings at each spot in the grid, in order to determine the resulting field amplitude for each zone.
\end{enumerate}

% is there something to cite about this MATLAB implementation?
%A simulator was first implemented in MATLAB on a version of the CBET problem that only calculated values for a 2-dimensional mesh. The implementations in the following sections were created based off of the MATLAB code, on the same 2-dimensional problem.
There are multiple academic teams and research facilities interested in tackling this problem using numerical models.
They implement various software programs and each has its own pros and cons.
Some examples are Lilac~\cite{Delettrez+:PRA87} DRACO~\cite{Radha+:POP05}, and Aster~\cite{Igumenshchev+:POP16}, and Hydra~\cite{Marinak+:POP96}.
Follett et al~\cite{Follett+:POP22} implemented the ray-based CBET model discussed in this paper first in MATLAB for expediency without consideration to performance.
It is able to consider multiple physics phenomena and produce accurate results, which are verified by comparing against other simulation tools.
However, due to limitations with the programming language and lack of software engineering practices during development, the MATLAB version is only capable of running small problems.
Also, it is difficult to scale the code to run on a server with hundreds of cores or even on accelerators. 
Therefore, it is important to study how modern programming language features could help in improving scalability and reducing errors when building large scientific programs like CBET.

\subsection{Rust}
Rust~\cite{KlabnikN:2017} is a programming language that takes some new approaches to certain problems in programming. Most important for this paper are its approaches to memory management and parallelism.

Memory management has traditionally been solved through manual memory management, as in C or C++, or through garbage collection, such as in MATLAB and Python. Garbage collection has significant performance costs, whereas manual memory management can introduce a lot of potential errors when not done carefully. Rust's approach is called the Ownership System. It prevents most of the errors manual memory management can create by enforcing a few rules on variables and references to them:

\begin{itemize}
    \item Each value (stored in memory) has exactly one owner variable. The memory is deallocated (dropped) when the owner goes out of scope. Ownership can be moved from one variable to another.
    \item Unlimited immutable references (also called borrows) can be made for any variable. However, as long as these immutable references are in scope, the memory they refer to cannot be mutated.
    \item One mutable reference (also called a mutable borrow) can be made for any variable. As long as this reference is in scope, the memory can only be read from or written to through that reference.
\end{itemize}

These are called ownership and borrow rules~\cite{KlabnikN:2017}.  Because these rules can be checked at compile-time, they offer solutions to memory problems that have no runtime cost. This makes Rust an attractive option for writing code where high-performance is needed, such as CBET. More language features that are useful to CBET are introduced in Sec~\ref{sec:impl:rust}.

==> old-sections/conclusion.tex <==
% !TEX root = main.tex 

\section{Conclusion}

We implement a simulation of the Cross Beam Energy Transfer interaction in C++ and in Rust, and compare their performance. Then, we measure the performance of a parallelized version of the Rust implementation that takes advantage of CPU multi-threading. We show that Rust can offer similar or even better performance for this task. Further, we show that parallel Rust code can be written easily and safely, with further performance gains. Thus, we argue that Rust is a strong contender for high performance scientific computing applications.

Future work for Rust in scientific computing could involve further comparisons between code written in Rust and in other programming languages, both for performance and for ease-of-use. However, Rust does not come without its limitations. For massively parallel workloads that may want to take advantage of GPUs with thousands of threads, Rust will fall short, not having native CUDA bindings. Furthermore, for Rust to be considered a more viable programming language in the scientific computing world, more libraries used in scientific computing should be written for Rust, or have Rust compatibility layers (as Rust has foreign function interfaces for C and C++).

There is more work to be done for CBET simulations as well, with the eventual goal of being able to simulate three-dimensional laser systems of dozens of lasers as efficiently as possible. The simulator computes intensities at one moment in time, so it must be able to run thousands of times with different mesh properties for each step of a full simulation of a laser system. In the future, optimizations for current implementations, as well as massively parallel implementations that take advantage of GPUs and multiple CPUs will be explored.

% Fill out with more conclusions and findings. 
% 
% For future work,
% massively parallel.
% GPUs?
% The OMEGA case requires 60 laser beams in 3D.
% The goal is to run a $\sim$2000x2000x2000 mesh ($\sim$10B zones) in as short a wall time as possible, since the algorithm computes the post-CBET laser intensities for just one snapshot in time. Thus, it must be run thousands of times with different mesh properties (electron density, temperature, flow velocity, etc.) for each step of the hydrodynamic simulation in order to model an entire implosion from the beginning of the laser drive through compression and stagnation of the target.


==> old-sections/impl.tex <==
% !TEX root = main.tex 

\section{Implementing CBET}
The following subsections describe the implementations of the CBET code in C++ and in Rust, noting the impacts of the programming language, as well as providing more details on how the rough outline described above was put into code.

\subsection{C++ Implementation}
\label{sec:impl:cpp}
The C++ version of CBET is implemented based on the MATLAB code written by Follett et al~\cite{Follett+:POP22,Follett+:PRE18}.
A laser beam to be launched into plasma is discretized by a set of initially parallel rays.
The computational modeling process involves two major steps of tracking rays across a mesh, which represents the plasma conditions (density, temperature, flow velocity, etc.).
%The first step is ray tracing, during which each ray is independently launched from its initial position and moves a small step at a prescribed short time interval until it exits the mesh.

The first major step is the ray tracing phase, wherein we must calculate the trajectory of each ray using coupled differential equations. There are several different forms the equations can take, but the form we chose and find to be most understandable is
\begin{equation}
\frac{d}{dt} \textbf{v} = -\frac{c^2}{2 n_{crit}} \nabla n_e
\end{equation}
\begin{equation}
\frac{d}{dt} \textbf{x} = \textbf{v}.
\end{equation} 
At each time step, the ray's position vector (\textbf{x}) is updated based on the velocity vector (\textbf{v}), whose calculation depends on the electron density gradient $\nabla n_e$ calculated at the current mesh location of the ray. The variable $c$ is the speed of light and $n_{crit}$ is the critical density of the plasma which depends on the wavelength of the laser light.
The dispersion relation that is enforced for transverse electromagnetic waves (i.e. laser light) is
\begin{equation}
\omega_L^2 = \omega_{p,e}^2 + c^2 k^2,
\end{equation}
where $\omega_L$ is the laser frequency, $\omega_{p,e}$ is the electron plasma frequency, and $k$ is the wavevector.
The wavevector, laser frequency, and velocity of the ray are related by the equation
\begin{equation}
\textbf{v} = c^2 \frac{\textbf{k}}{\omega_L}.
\end{equation}
The net result of this process is that each of the many rays representing each laser beam is marched across the mesh. Typically each ray travels in slightly different directions with slightly different headings and velocities. The entire path traced out is called the ray's trajectory, which typically bends (i.e. refracts) in the presence of the electron density gradient. Each ray trajectory calculation is independent of the others and so this phase should be embarassingly parallel. 
After every ray exits the mesh, we have a complete trajectory for each ray.
We can also derive other important values from the ray trajectories, such as \textbf{k} vectors when rays enter new zones.
These values will be used to calculate the CBET in the second step.
We also launch an ``auxiliary" ray (or child ray) with a slight offset compared to the corresponding main ray (or parent ray).
The child ray has the same intensity and initial \textbf{k} vector as its parent ray.
As both rays go through the plasma, the subtle difference in initial position will give them a slightly different velocity at each time step, and therefore the trajectories are not perfectly parallel.
The change in separation distance between main ray and auxiliary ray represent the change in the laser beam's intensity, $I_L$ [W/m$^{2}$]. A laser's intensity is related to its electric field strength $E$ [V/m] through the relation 
\begin{equation}
I_L = \frac{1}{2} \epsilon_0 c E^2
\end{equation}
where $\epsilon_0$ is the permittivity of free space. An equivalent way of characterizing the strength of the laser field is the normalized vector potential
\begin{equation}
a_0 = \frac{e E}{m_e c \omega_L} = \sqrt{\frac{2 I_L}{\epsilon_0 c^3}} \frac{e}{m_e \omega_L}
\end{equation}
where $e$ and $m_e$ are the charge and mass of the electron, respectively. As equation (6) illustrates, $a_0$, $E$, and $I_L$ are all related and interchangeable when discussing the electromagnetic field strength of the laser.

The second major step is the CBET calculation itself, which is responsible for evaluating the redirection of laser intensity or energy among the rays making up each laser beam.
Based on the trajectories obtained from step one, if two rays enter the same zone, they are considered to intersect, and therefore energy can be exchanged.
The overall CBET calculation step is implemented as an iterative procedure: for each ray, the code iterates over all possible intersections, calculates the CBET coupling multiplier for energy exchange, and propagates the result of the energy change to the remaining downstream portion of the trajectory.
The process is repeated until the solution converges, meaning the answer stops changing with additional iterations (i.e, the maximum amount of relative energy exchange within a single iteration is below a predefined, small threshold; typical values might be 1e-3 to 1e-4).
%The energy is exchanged among rays that intersect within the same zone until a steady state is reached.

Although the C++ version is not fully-optimized, rewriting CBET code from MATLAB to C++ enables the possibility of exploring different research directions, such as this comparison with Rust.
To make a fair comparison, the C++ version used in Sec~\ref{sec:perf} is modified to be more similar to the Rust implementation as described in Sec~\ref{sec:impl:rust}. However, the structure of the data is different in some cases.

\begin{figure}
\includegraphics[width=0.49\textwidth]{figure.jpg}
    \caption{Test cases of the 2D 2-beam and 3-beam CBET problem using different initial laser intensities. All plots and lineouts are in the dimensionless units of the normalized vector potential $a_0$. The beam moving from bottom-to-top transfers its energy to the beam(s) moving from left-to-right.}
    \label{fig:SAMM-basics}
\end{figure}

\subsection{Rust Implementation}
\label{sec:impl:rust}

The Rust implementation of the CBET program was created after the C++ implementation, and was heavily based off the C++ code. The methods for performing the calculation are the same, but the design of the Rust implementation is somewhat different, taking advantage of Rust's modularity features. Rust treats each source code file as a module, which is given its own namespace when referenced by other parts of code. The main source code file is short and only calls into these various modules. By moving as much code as possible into modules, we can upload the CBET code to Rust's package repositories in the future, for others to use.

Some important language features used in the Rust program are iterators and closures.  An \emph{iterator} is a control abstraction for performing a task on a sequence of items~\cite[Chapter 13]{KlabnikN:2017}.  The task is written in an anonymous function, which is a first-class value that can be created dynamically based on variable values in a running function, returned from the function, or passed as a parameter when calling another function~\cite{Scott:PLPv4}.  In Rust, anonymous functions are implemented as and called closures.

While a C++ programmer typically writes a loop including both looping control and data processing, a Rust programmer typically calls an iterator method supplying a closure.  The latter avoids repeating control code and improves code reuse and correctness.  
Once a collection is turned into an iterator, it can be adapted with methods such as ``map'', or consumed with methods such as ``fold'' and ``reduce''. Iterator methods are lazy, meaning that they do not do anything until they are consumed. 
Unlike in previous functional languages, in Rust iterators are implemented with very little overhead compared to loops~\cite[Chapter 13]{KlabnikN:2017}.  Later we will evaluate the cost of using iterators and closures in CBET.  

% (CD) This is not necessarily true: Iterators also erase the runtime overhead of bounds checking on collections. 

In Rust, the ownership and borrowing system is also enforced on closures, and functions can specify whether or not the closure can borrow references from their environment, mutably or immutably, in their type signature. This feature, in addition to contributing to memory safety, also makes parallelism easier, as functions which execute in parallel can specify that they can't borrow mutable references from their environment (which could cause data races), and code that does so will not compile.

An example of the use of iterators and closures in the CBET program can be found in Fig~\ref{fig:seq_iter_ex}, which shows an excerpt from the ray tracing part of the code. In this example, the ``beams'' variable refers to a vector of beam structs. The ``iter\_mut'' method on the vector transforms it into an iterator, where each reference in the iterator is mutable. Then, the ``for\_each'' method runs the closure it is provided on each element of the iterator. The third line initializes the marked array, which contains a vector for each zone in the mesh. It does so by creating a range, which is a type of iterator, and then using the ``map'' adapter to change each element in the range into an empty vector. Finally, the ``collect'' iterator method turns the iterator into a collection, here a vector. The following lines iterate over the rays of the beam in a similar way, with the ``enumerate'' adapter turning each element of the iterator into a tuple containing the index of the element and that element.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/seq_iter_ex.png}
    \caption{Rust Example: Iterators and Closures}
    \label{fig:seq_iter_ex}
\end{figure}

Rust was built from the ground up to support safe concurrency. In order to explore the use of parallel code in Rust, a version of the Rust implementation was made that takes advantage of CPU-based multi-threading. The multi-threading is implemented using the Rayon library~\cite{Rayon}. Rayon builds on top of the Rust standard library's threading features to make parallel code easier to write and faster to execute. It creates a thread pool, and uses a work-stealing algorithm to distribute work evenly. While this creates a little bit of runtime overhead, as we show, the performance benefits of using Rayon in our CBET implementation are still great.

Using the library can be as simple as replacing the use of methods which turn collections into iterators with Rayon's implementations, which turn collections into parallel iterators. Then, the methods implemented on the iterators, such as ``map'' and ``for\_each'', are run in parallel. The ease of this conversion is aided by the aforementioned rules around the closures that the iterator methods take. Rayon can specify in its function headers that the closures it takes must be thread-safe, and then the Rust compiler will refuse to compile code that isn't thread safe, drastically reducing the potential for thread-related errors such as data races.

Sometimes, Rust's ownership and borrowing rules prevent some types of valid memory uses. For example, multiple threads may need to write to the same section of memory, but in thread-safe Rust code, mutable references may not be used in threads. In order to remedy this, Rust introduces Smart Pointers, which enforce the borrow checking rules at run-time instead of compile-time. One such smart pointer that is used in the parallel CBET implementation is the Mutex, which allows only one thread to read from or write to the memory it owns at any given time. Mutexes can be passed as immutable references to the closures that execute in parallel, and when they are locked, they give the thread access to a mutable reference to the memory inside.

An example of the parallel CBET code can be seen in Fig~\ref{fig:par_iter_ex}, which is the modified version of the earlier example in Fig~\ref{fig:seq_iter_ex}. Here, the iterator over the rays of each beam is modified to use Rayon's ``par\_iter\_mut'' method. Then, because the closure in the sequential code borrowed a reference to the marked array mutably, and that is not thread-safe, the borrow in the parallel code is not mutable, and instead Mutexes are used for memory that needs to be written to from multiple threads, a change that is reflected in the third line of the example.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/par_iter_ex.png}
    \caption{Rust Example: Parallel Iterators}
    \label{fig:par_iter_ex}
\end{figure}

In order to keep the comparison as direct as possible, no optimizations were made to the sequential Rust code besides using Rayon's parallel iterators and making the necessary modifications (such as adding Mutexes and modifying code to prevent writing to the same memory in multiple threads). The subroutines that were parallelized include ray tracing and the step of the CBET process that calculates the interaction multiplier. The difference between the sequential and parallel versions is only 67 Source Lines of Code, as calculated from the git diff.

==> old-sections/intro.tex <==
% !TEX root = main.tex 

\section{Introduction}

As the field of computational science continues to grow, demand increases for the use of high-performance scientific computation, which enables faster modeling of more complex interactions and analysis of larger datasets. A survey of computational scientists across a wide range of disciplines conducted by Princeton University found that close to 1/4 of the scientists use programming languages like C and C++ in order to write performance-intensive computation code~\cite{Prabhu+:SC11}.
% cite a source for why c/c++ are faster than matlab/python? and think of something better than "because they are compiled"
% perhaps something like "c and c++ are used for a variety of reasons..."
Unlike MATLAB and Python, C and C++ are compiled and rely on manual memory management rather than garbage collection, offering the greater performance needed in certain applications. They are established programming languages, having been around for several decades, with numerous libraries and tools written for various computational science applications.
% cite a source for Rust provides similar performance to c/c++?
% by "code complexity" I mean how easy it is to write/read code in Rust, maybe that could be reworded?
Rust is a relative newcomer in the programming language space. It offers similar performance to languages such as C and C++, but takes a variety of new approaches to solve problems such as memory safety and parallelism, making it a great choice for computational scientists.

% perhaps cite a source for what CBET is?
This paper looks at the benefits of Rust through the re-implementation of a simulation of laser-plasma interaction from C++ to Rust. Specifically, Cross Beam Energy Transfer (CBET) effect happens when high-intensity laser beams intersect in a plasma. The measurable outcome of the interaction is a change in the beams' intensities, i.e. how much energy is present in each participating laser beam after the interaction is calculated. Simulating this interaction is a crucial step in building an accurate simulator of laser systems in order to aid research on topics such as inertial confinement nuclear fusion, high-energy-density physics, materials science, laboratory astrophysics, and fundamental science. 

==> old-sections/related.tex <==
% !TEX root = main.tex 

\section{Related Work}

There are a few works that explore the benefit of using Rust for HPC applications.
Costanzo et al.~\cite{Costanzo+:CLEI21} study a scientific application named N-body, and find that Rust greatly reduce programming effort while providing similar performance compared to C.
They find that Rust is easier to be parallelized, has better readability, and needs fewer lines of code to express the same functionality.
Rotter et al.~\cite{Rotter+:CSCI22} further analyze a special implementation of N-body problem, and find that while C/C++ version takes less time to finish for small problems, Rust potentially has better scalability at large problem scale. This finding is consistent with our findings, as the performance improvement of Rust over C++ is greater in the larger problem case.
%Here we will discuss some of them in the context of our work. Similar or dissimilar findings?


==> old-sections/result.tex <==
% !TEX root = main.tex 

\section{Performance Results}
\label{sec:perf}

\subsection{Machine Specifications}
\label{sec:result:machine}

We ran the different implementations on three machines. They have been sorted in chronological order by processor, with the newest processors at the end. The Rust compiler version is 1.79.0 on all machines. The first machine, referred to as Xeon, has the following specifications:

\begin{itemize}
    \item Intel Xeon W-2295 CPU
    \item Base frequency of 3.00 GHz, with boost up to 4.80 GHz
    \item 18 cores, 36 threads
    \item 24.75 MB L3 Cache
    \item 256 GB of memory
    \item C++ code compiled by GCC 11.4.0
\end{itemize}

The second machine, referred to as Threadripper, has the following specifications:
\begin{itemize}
    \item AMD Ryzen Threadripper PRO 5975WX CPU
    \item Base frequency of 3.6 GHz, with boost up to 4.5 GHz
    \item 32 cores, 64 threads
    \item 128 MB L3 Cache
    \item 128 GB of memory
    \item C++ code compiled by GCC 12.3.0
\end{itemize}

The third machine, referred to as EPYC, has the following specifications:
\begin{itemize}
    \item AMD EPYC 9124 CPU
    \item Base frequency of 3.00 GHz, with boost up to 3.7 GHz
    \item 16 cores, 32 threads
    \item 64 MB L3 Cache
    \item 192 GB of memory
    \item C++ code compiled by GCC 11.4.0
\end{itemize}

\subsection{Sequential Comparison}

We tested the C++ and Rust implementations of CBET, simulating the interaction of two high-intensity laser beams in a two-dimensional mesh. The implementations were compiled with -O3 optimizations, and the Rust implementation was run with one thread, to make a fair sequential comparison. Figure~\ref{fig:seq:500} shows the performance results when simulating on a mesh with 500 zones in each dimension, and Figure~\ref{fig:seq:2500} shows the performance results when simulating on a mesh with 2500 zones in each dimension.

These results show that our Rust implementation is at least twice as fast as the C++ implementation, with performance gains of up to 6.67$\times$, in the case of the large mesh on the EPYC machine. Thus, the high level abstractions discussed in Sec~\ref{sec:impl:rust} come at a low enough performance cost to be viable in high-performance computing applications.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/seq 500.png}
    \caption{CBET sequential version runtime for 500 $\times$ 500 mesh}
    \label{fig:seq:500}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/seq 2500.png}
    \caption{CBET sequential version runtime for 2500 $\times$ 2500 mesh}
    \label{fig:seq:2500}
\end{figure}

We think the following reasons may explain some of the differences in performance.  First, Rust code uses mainly structs, while the C++ code uses arrays.  This leads to a different data layout which may affect memory performance.  Second, lazy iterator methods in Rust allow computations on the same data to be combined and may have better cache performance.  For example, in map followed by sum, the processing and summing are done in a single pass of data.

\subsection{Parallel Rust}

Table~\ref{tab:parallel} shows the execution time of the parallel version on the same machines used above, with the same problem that the sequential versions of the simulator are tested with. By default, Rayon uses the number of logical threads that are provided, so for Xeon, Threadripper, and EPYC, the number of threads are 36, 64, and 32 respectively. In order to test the strong scaling performance of the various machines available, we also tested the problem, for both mesh sizes, at different numbers of threads in the thread pool (capped at 32 threads). Figure~\ref{fig:strong-scaling-2500} shows the strong scaling performance of the simulator relative to using single thread on Xeon machine.

\begin{table}[h!]
\caption{Rust parallel version runtime}
\begin{center}
    \begin{tabular}{ |c|c|c| }
        \hline
        machine & 500x500 & 2500x2500 \\
        \hline
        Xeon & 1.344s & 24.926s \\
        \hline
        Threadripper & 1.313s & 17.727s \\
        \hline
        EPYC & 1.347 & 15.600s \\
        \hline
    \end{tabular}
\label{tab:parallel}
\end{center}
\end{table}


% https://docs.google.com/spreadsheets/d/1RC25dV1rBXats5U8j10kW7el_r4OqQEZuwEkVb-V3PI/edit?usp=sharing
begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/strong scaling 2500.png}
    \caption{Multi-Threaded Performance on a 2500x2500 Mesh}
    \label{fig:strong-scaling-2500}
\end{figure}

